On the Energy Footprint of Mobile Testing Frameworks

High energy consumption is a challenging issue that an ever increasing number of mobile applications face today. However, energy consumption is being tested in an ad hoc way, despite being an important non-functional requirement of an application. Such limitation becomes particularly disconcerting during software testing: on the one hand, developers do not really know how to measure energy; on the other hand, there is no knowledge as to what is the energy overhead imposed by the testing framework. In this paper, as we evaluate eight popular mobile UI automation frameworks, we have discovered that there are automation frameworks that increase energy consumption up to roughly 2200%. While limited in the interactions one can do, Espresso is the most energy efficient framework. However, depending on the needs of the tester, Appium, Monkeyrunner, or UIAutomator are good alternatives. In practice, results show that deciding which is the most suitable framework is vital. We provide a decision tree to help developers make an educated decision on which framework suits best their testing needs.

==> results/overheads_summary.tex <==
\begin{tabular}{llllllll}
\hline
                   & Tap     & Swipe   & Back Button   & Dragndrop   & Input Text   & Pinch And Spread   & Long Tap   \\
\hline
 AndroidViewClient & 274.6\% & 421.7\% & 439.7\%       & 211.1\%     & 935.7\%      & n.a.               & 274.6\%    \\
 Appium            & 870.8\% & 154.8\% & -81.2\%       & 798.9\%     & 106.3\%      & n.a.               & 124.3\%    \\
 Calabash          & 470.2\% & 469.9\% & 63.9\%        & 2193.0\%    & 29.0\%       & 374.0\%            & 309.5\%    \\
 Espresso          & 15.6\%  & 29.2\%  & -76.6\%       & n.a.        & -64.9\%      & n.a.               & 80.9\%     \\
 Monkeyrunner      & 175.2\% & 427.5\% & -88.8\%       & 501.1\%     & -60.8\%      & n.a.               & 77.1\%     \\
 PythonUiAutomator & 77.6\%  & 259.1\% & 25.5\%        & 505.4\%     & -63.3\%      & 180.6\%            & 308.6\%    \\
 Robotium          & 210.5\% & 416.4\% & -76.9\%       & 250.2\%     & -80.9\%      & n.a.               & 187.4\%    \\
 UiAutomator       & 36.5\%  & 261.2\% & 9.7\%         & 184.8\%     & -88.1\%      & -5.0\%             & 94.0\%     \\
\hline
\end{tabular}

==> results/table_ranking.tex <==
\begin{tabular}{lr}
\hline
 Framework         &   Score \\
\hline
 UiAutomator       &  6.2698 \\
 Espresso          &  5.3135 \\
 Human             &  4.8194 \\
 Robotium          &  4.6766 \\
 PythonUiAutomator &  3.8214 \\
 Monkeyrunner      &  3.6667 \\
 Appium            &  3.2619 \\
 AndroidViewClient &  1.7262 \\
 Calabash          &  0.4444 \\
\hline
\end{tabular}

==> results/table_welchsttest_back_button.tex <==
\begin{tabular}{llllllllll}
\hline
                   & Human                  & AndroidViewClient       & Appium                 & Calabash                & Espresso                & Monkeyrunner           & PythonUiAutomator     & Robotium               & UiAutomator   \\
\hline
 Human             & --                     & --                      & --                     & --                      & --                      & --                     & --                    & --                     & --            \\
 AndroidViewClient & (test=106.71, p\ensuremath{<}0.001) & --                      & --                     & --                      & --                      & --                     & --                    & --                     & --            \\
 Appium            & (test=-30.79, p\ensuremath{<}0.001) & (test=-212.35, p\ensuremath{<}0.001) & --                     & --                      & --                      & --                     & --                    & --                     & --            \\
 Calabash          & (test=25.05, p\ensuremath{<}0.001)  & (test=-131.69, p\ensuremath{<}0.001) & (test=196.11, p\ensuremath{<}0.001) & --                      & --                      & --                     & --                    & --                     & --            \\
 Espresso          & (test=-17.85, p\ensuremath{<}0.001) & (test=-194.60, p\ensuremath{<}0.001) & (test=102.74, p\ensuremath{<}0.001) & (test=-144.88, p\ensuremath{<}0.001) & --                      & --                     & --                    & --                     & --            \\
 Monkeyrunner      & (test=-31.99, p\ensuremath{<}0.001) & (test=-214.16, p\ensuremath{<}0.001) & (test=-15.25, p\ensuremath{<}0.001) & (test=-202.30, p\ensuremath{<}0.001) & (test=-118.99, p\ensuremath{<}0.001) & --                     & --                    & --                     & --            \\
 PythonUiAutomator & (test=59.46, p\ensuremath{<}0.001)  & (test=-62.72, p\ensuremath{<}0.001)  & (test=154.02, p\ensuremath{<}0.001) & (test=62.95, p\ensuremath{<}0.001)   & (test=133.35, p\ensuremath{<}0.001)  & (test=156.10, p\ensuremath{<}0.001) & --                    & --                     & --            \\
 Robotium          & (test=39.20, p\ensuremath{<}0.001)  & (test=-24.36, p\ensuremath{<}0.001)  & (test=60.24, p\ensuremath{<}0.001)  & (test=30.31, p\ensuremath{<}0.001)   & (test=53.47, p\ensuremath{<}0.001)   & (test=60.87, p\ensuremath{<}0.001)  & (test=6.70, p\ensuremath{<}0.001)  & --                     & --            \\
 UiAutomator       & (test=59.61, p\ensuremath{<}0.001)  & (test=-82.49, p\ensuremath{<}0.001)  & (test=245.93, p\ensuremath{<}0.001) & (test=79.64, p\ensuremath{<}0.001)   & (test=206.86, p\ensuremath{<}0.001)  & (test=250.48, p\ensuremath{<}0.001) & (test=-9.82, p\ensuremath{<}0.001) & (test=-10.77, p\ensuremath{<}0.001) & --            \\
\hline
\end{tabular}


==> results/table_welchsttest_dragndrop.tex <==
\begin{tabular}{lllllllll}
\hline
                   & Human                  & AndroidViewClient      & Appium                  & Calabash                & Monkeyrunner           & PythonUiAutomator      & Robotium               & UiAutomator   \\
\hline
 Human             & --                     & --                     & --                      & --                      & --                     & --                     & --                     & --            \\
 AndroidViewClient & (test=36.63, p\ensuremath{<}0.001)  & --                     & --                      & --                      & --                     & --                     & --                     & --            \\
 Appium            & (test=88.66, p\ensuremath{<}0.001)  & (test=88.06, p\ensuremath{<}0.001)  & --                      & --                      & --                     & --                     & --                     & --            \\
 Calabash          & (test=169.77, p\ensuremath{<}0.001) & (test=167.40, p\ensuremath{<}0.001) & (test=130.56, p\ensuremath{<}0.001)  & --                      & --                     & --                     & --                     & --            \\
 Monkeyrunner      & (test=49.50, p\ensuremath{<}0.001)  & (test=25.83, p\ensuremath{<}0.001)  & (test=-47.48, p\ensuremath{<}0.001)  & (test=-150.56, p\ensuremath{<}0.001) & --                     & --                     & --                     & --            \\
 PythonUiAutomator & (test=36.79, p\ensuremath{<}0.001)  & (test=21.01, p\ensuremath{<}0.001)  & (test=-10.15, p\ensuremath{<}0.001)  & (test=-101.78, p\ensuremath{<}0.001) & (test=10.55, p\ensuremath{<}0.001)  & --                     & --                     & --            \\
 Robotium          & (test=32.97, p\ensuremath{<}0.001)  & (test=-2.90, p=0.005)  & (test=-81.14, p\ensuremath{<}0.001)  & (test=-165.48, p\ensuremath{<}0.001) & (test=-25.72, p\ensuremath{<}0.001) & (test=-21.62, p\ensuremath{<}0.001) & --                     & --            \\
 UiAutomator       & (test=18.85, p\ensuremath{<}0.001)  & (test=-37.40, p\ensuremath{<}0.001) & (test=-120.68, p\ensuremath{<}0.001) & (test=-178.73, p\ensuremath{<}0.001) & (test=-52.48, p\ensuremath{<}0.001) & (test=-30.77, p\ensuremath{<}0.001) & (test=-27.61, p\ensuremath{<}0.001) & --            \\
\hline
\end{tabular}


==> results/table_welchsttest_find_by_content.tex <==
\begin{tabular}{llllllll}
\hline
                   & AndroidViewClient       & Appium                 & Calabash               & Espresso               & PythonUiAutomator      & Robotium                & UiAutomator   \\
\hline
 AndroidViewClient & --                      & --                     & --                     & --                     & --                     & --                      & --            \\
 Appium            & (test=-108.47, p\ensuremath{<}0.001) & --                     & --                     & --                     & --                     & --                      & --            \\
 Calabash          & (test=-5.60, p\ensuremath{<}0.001)   & (test=33.25, p\ensuremath{<}0.001)  & --                     & --                     & --                     & --                      & --            \\
 Espresso          & (test=-76.81, p\ensuremath{<}0.001)  & (test=33.01, p\ensuremath{<}0.001)  & (test=-25.37, p\ensuremath{<}0.001) & --                     & --                     & --                      & --            \\
 PythonUiAutomator & (test=-109.48, p\ensuremath{<}0.001) & (test=0.40, p=0.688)   & (test=-33.27, p\ensuremath{<}0.001) & (test=-33.77, p\ensuremath{<}0.001) & --                     & --                      & --            \\
 Robotium          & (test=-41.15, p\ensuremath{<}0.001)  & (test=194.00, p\ensuremath{<}0.001) & (test=-9.27, p\ensuremath{<}0.001)  & (test=69.87, p\ensuremath{<}0.001)  & (test=212.88, p\ensuremath{<}0.001) & --                      & --            \\
 UiAutomator       & (test=-101.86, p\ensuremath{<}0.001) & (test=3.34, p=0.002)   & (test=-32.53, p\ensuremath{<}0.001) & (test=-27.25, p\ensuremath{<}0.001) & (test=3.33, p=0.002)   & (test=-137.81, p\ensuremath{<}0.001) & --            \\
\hline
\end{tabular}


==> results/table_welchsttest_find_by_description.tex <==
\begin{tabular}{lllllll}
\hline
                   & AndroidViewClient       & Appium                 & Calabash               & Espresso              & PythonUiAutomator      & UiAutomator   \\
\hline
 AndroidViewClient & --                      & --                     & --                     & --                    & --                     & --            \\
 Appium            & (test=-169.04, p\ensuremath{<}0.001) & --                     & --                     & --                    & --                     & --            \\
 Calabash          & (test=3.48, p=0.002)    & (test=26.76, p\ensuremath{<}0.001)  & --                     & --                    & --                     & --            \\
 Espresso          & (test=-243.11, p\ensuremath{<}0.001) & (test=-46.36, p\ensuremath{<}0.001) & (test=-30.72, p\ensuremath{<}0.001) & --                    & --                     & --            \\
 PythonUiAutomator & (test=-176.37, p\ensuremath{<}0.001) & (test=1.48, p=0.144)   & (test=-26.63, p\ensuremath{<}0.001) & (test=56.05, p\ensuremath{<}0.001) & --                     & --            \\
 UiAutomator       & (test=-173.05, p\ensuremath{<}0.001) & (test=-8.20, p\ensuremath{<}0.001)  & (test=-27.73, p\ensuremath{<}0.001) & (test=33.07, p\ensuremath{<}0.001) & (test=-10.21, p\ensuremath{<}0.001) & --            \\
\hline
\end{tabular}


==> results/table_welchsttest_find_by_id.tex <==
\begin{tabular}{lllllllll}
\hline
                   & AndroidViewClient       & Appium                 & Calabash                & Espresso               & Monkeyrunner           & PythonUiAutomator     & Robotium                & UiAutomator   \\
\hline
 AndroidViewClient & --                      & --                     & --                      & --                     & --                     & --                    & --                      & --            \\
 Appium            & (test=-99.14, p\ensuremath{<}0.001)  & --                     & --                      & --                     & --                     & --                    & --                      & --            \\
 Calabash          & (test=7.47, p\ensuremath{<}0.001)    & (test=88.53, p\ensuremath{<}0.001)  & --                      & --                     & --                     & --                    & --                      & --            \\
 Espresso          & (test=-118.57, p\ensuremath{<}0.001) & (test=-47.31, p\ensuremath{<}0.001) & (test=-102.80, p\ensuremath{<}0.001) & --                     & --                     & --                    & --                      & --            \\
 Monkeyrunner      & (test=-105.21, p\ensuremath{<}0.001) & (test=-19.97, p\ensuremath{<}0.001) & (test=-94.27, p\ensuremath{<}0.001)  & (test=10.46, p\ensuremath{<}0.001)  & --                     & --                    & --                      & --            \\
 PythonUiAutomator & (test=-35.05, p\ensuremath{<}0.001)  & (test=3.18, p=0.003)   & (test=-37.93, p\ensuremath{<}0.001)  & (test=9.11, p\ensuremath{<}0.001)   & (test=7.24, p\ensuremath{<}0.001)   & --                    & --                      & --            \\
 Robotium          & (test=-30.23, p\ensuremath{<}0.001)  & (test=172.95, p\ensuremath{<}0.001) & (test=-33.39, p\ensuremath{<}0.001)  & (test=303.19, p\ensuremath{<}0.001) & (test=162.76, p\ensuremath{<}0.001) & (test=25.15, p\ensuremath{<}0.001) & --                      & --            \\
 UiAutomator       & (test=-94.32, p\ensuremath{<}0.001)  & (test=-3.73, p\ensuremath{<}0.001)  & (test=-86.13, p\ensuremath{<}0.001)  & (test=24.64, p\ensuremath{<}0.001)  & (test=12.40, p\ensuremath{<}0.001)  & (test=-4.00, p\ensuremath{<}0.001) & (test=-127.44, p\ensuremath{<}0.001) & --            \\
\hline
\end{tabular}


==> results/table_welchsttest_input_text.tex <==
\begin{tabular}{llllllllll}
\hline
                   & Human                  & AndroidViewClient       & Appium                  & Calabash                & Espresso               & Monkeyrunner           & PythonUiAutomator     & Robotium              & UiAutomator   \\
\hline
 Human             & --                     & --                      & --                      & --                      & --                     & --                     & --                    & --                    & --            \\
 AndroidViewClient & (test=181.77, p\ensuremath{<}0.001) & --                      & --                      & --                      & --                     & --                     & --                    & --                    & --            \\
 Appium            & (test=26.84, p\ensuremath{<}0.001)  & (test=-203.13, p\ensuremath{<}0.001) & --                      & --                      & --                     & --                     & --                    & --                    & --            \\
 Calabash          & (test=6.46, p\ensuremath{<}0.001)   & (test=-236.71, p\ensuremath{<}0.001) & (test=-43.33, p\ensuremath{<}0.001)  & --                      & --                     & --                     & --                    & --                    & --            \\
 Espresso          & (test=-20.25, p\ensuremath{<}0.001) & (test=-268.43, p\ensuremath{<}0.001) & (test=-106.75, p\ensuremath{<}0.001) & (test=-105.01, p\ensuremath{<}0.001) & --                     & --                     & --                    & --                    & --            \\
 Monkeyrunner      & (test=-21.08, p\ensuremath{<}0.001) & (test=-268.84, p\ensuremath{<}0.001) & (test=-107.77, p\ensuremath{<}0.001) & (test=-105.72, p\ensuremath{<}0.001) & (test=-10.17, p\ensuremath{<}0.001) & --                     & --                    & --                    & --            \\
 PythonUiAutomator & (test=-11.73, p\ensuremath{<}0.001) & (test=-187.21, p\ensuremath{<}0.001) & (test=-40.07, p\ensuremath{<}0.001)  & (test=-21.67, p\ensuremath{<}0.001)  & (test=2.88, p=0.007)   & (test=3.68, p\ensuremath{<}0.001)   & --                    & --                    & --            \\
 Robotium          & (test=-22.68, p\ensuremath{<}0.001) & (test=-266.10, p\ensuremath{<}0.001) & (test=-103.17, p\ensuremath{<}0.001) & (test=-90.29, p\ensuremath{<}0.001)  & (test=-13.39, p\ensuremath{<}0.001) & (test=-9.13, p\ensuremath{<}0.001)  & (test=-5.50, p\ensuremath{<}0.001) & --                    & --            \\
 UiAutomator       & (test=-24.08, p\ensuremath{<}0.001) & (test=-260.44, p\ensuremath{<}0.001) & (test=-95.42, p\ensuremath{<}0.001)  & (test=-75.62, p\ensuremath{<}0.001)  & (test=-15.04, p\ensuremath{<}0.001) & (test=-12.37, p\ensuremath{<}0.001) & (test=-7.35, p\ensuremath{<}0.001) & (test=-5.62, p\ensuremath{<}0.001) & --            \\
\hline
\end{tabular}


==> results/table_welchsttest_long_tap.tex <==
\begin{tabular}{llllllllll}
\hline
                   & Human                 & AndroidViewClient      & Appium                 & Calabash               & Espresso              & Monkeyrunner          & PythonUiAutomator      & Robotium               & UiAutomator   \\
\hline
 Human             & --                    & --                     & --                     & --                     & --                    & --                    & --                     & --                     & --            \\
 AndroidViewClient & (test=34.33, p\ensuremath{<}0.001) & --                     & --                     & --                     & --                    & --                    & --                     & --                     & --            \\
 Appium            & (test=29.20, p\ensuremath{<}0.001) & (test=-24.17, p\ensuremath{<}0.001) & --                     & --                     & --                    & --                    & --                     & --                     & --            \\
 Calabash          & (test=66.46, p\ensuremath{<}0.001) & (test=-2.16, p=0.037)  & (test=58.11, p\ensuremath{<}0.001)  & --                     & --                    & --                    & --                     & --                     & --            \\
 Espresso          & (test=16.72, p\ensuremath{<}0.001) & (test=-29.96, p\ensuremath{<}0.001) & (test=-28.96, p\ensuremath{<}0.001) & (test=-77.38, p\ensuremath{<}0.001) & --                    & --                    & --                     & --                     & --            \\
 Monkeyrunner      & (test=20.75, p\ensuremath{<}0.001) & (test=-27.97, p\ensuremath{<}0.001) & (test=-17.27, p\ensuremath{<}0.001) & (test=-69.67, p\ensuremath{<}0.001) & (test=10.70, p\ensuremath{<}0.001) & --                    & --                     & --                     & --            \\
 PythonUiAutomator & (test=14.67, p\ensuremath{<}0.001) & (test=-0.39, p=0.698)  & (test=9.72, p\ensuremath{<}0.001)   & (test=0.52, p=0.606)   & (test=12.06, p\ensuremath{<}0.001) & (test=11.28, p\ensuremath{<}0.001) & --                     & --                     & --            \\
 Robotium          & (test=51.21, p\ensuremath{<}0.001) & (test=-9.54, p\ensuremath{<}0.001)  & (test=37.37, p\ensuremath{<}0.001)  & (test=-15.96, p\ensuremath{<}0.001) & (test=55.16, p\ensuremath{<}0.001) & (test=48.29, p\ensuremath{<}0.001) & (test=-3.73, p\ensuremath{<}0.001)  & --                     & --            \\
 UiAutomator       & (test=22.45, p\ensuremath{<}0.001) & (test=-27.25, p\ensuremath{<}0.001) & (test=-13.85, p\ensuremath{<}0.001) & (test=-67.56, p\ensuremath{<}0.001) & (test=14.67, p\ensuremath{<}0.001) & (test=3.58, p\ensuremath{<}0.001)  & (test=-10.98, p\ensuremath{<}0.001) & (test=-46.26, p\ensuremath{<}0.001) & --            \\
\hline
\end{tabular}


==> results/table_welchsttest_multi_finger_tap.tex <==
\begin{tabular}{ll}
\hline
        & Appium   \\
\hline
 Appium & --       \\
\hline
\end{tabular}


==> results/table_welchsttest_pinch_and_spread.tex <==
\begin{tabular}{lllll}
\hline
                   & Human                 & Calabash               & PythonUiAutomator      & UiAutomator   \\
\hline
 Human             & --                    & --                     & --                     & --            \\
 Calabash          & (test=19.47, p\ensuremath{<}0.001) & --                     & --                     & --            \\
 PythonUiAutomator & (test=48.59, p\ensuremath{<}0.001) & (test=-9.18, p\ensuremath{<}0.001)  & --                     & --            \\
 UiAutomator       & (test=-1.00, p=0.322) & (test=-19.61, p\ensuremath{<}0.001) & (test=-44.79, p\ensuremath{<}0.001) & --            \\
\hline
\end{tabular}


==> results/table_welchsttest_swipe.tex <==
\begin{tabular}{llllllllll}
\hline
                   & Human                  & AndroidViewClient       & Appium                 & Calabash                & Espresso               & Monkeyrunner           & PythonUiAutomator     & Robotium               & UiAutomator   \\
\hline
 Human             & --                     & --                      & --                     & --                      & --                     & --                     & --                    & --                     & --            \\
 AndroidViewClient & (test=151.27, p\ensuremath{<}0.001) & --                      & --                     & --                      & --                     & --                     & --                    & --                     & --            \\
 Appium            & (test=35.27, p\ensuremath{<}0.001)  & (test=-197.70, p\ensuremath{<}0.001) & --                     & --                      & --                     & --                     & --                    & --                     & --            \\
 Calabash          & (test=132.37, p\ensuremath{<}0.001) & (test=-10.69, p\ensuremath{<}0.001)  & (test=151.81, p\ensuremath{<}0.001) & --                      & --                     & --                     & --                    & --                     & --            \\
 Espresso          & (test=5.75, p\ensuremath{<}0.001)   & (test=-281.09, p\ensuremath{<}0.001) & (test=-69.21, p\ensuremath{<}0.001) & (test=-208.87, p\ensuremath{<}0.001) & --                     & --                     & --                    & --                     & --            \\
 Monkeyrunner      & (test=79.40, p\ensuremath{<}0.001)  & (test=-28.98, p\ensuremath{<}0.001)  & (test=67.70, p\ensuremath{<}0.001)  & (test=-21.14, p\ensuremath{<}0.001)  & (test=93.86, p\ensuremath{<}0.001)  & --                     & --                    & --                     & --            \\
 PythonUiAutomator & (test=64.30, p\ensuremath{<}0.001)  & (test=-92.50, p\ensuremath{<}0.001)  & (test=49.42, p\ensuremath{<}0.001)  & (test=-74.61, p\ensuremath{<}0.001)  & (test=91.67, p\ensuremath{<}0.001)  & (test=-31.57, p\ensuremath{<}0.001) & --                    & --                     & --            \\
 Robotium          & (test=131.76, p\ensuremath{<}0.001) & (test=-23.52, p\ensuremath{<}0.001)  & (test=160.23, p\ensuremath{<}0.001) & (test=-10.09, p\ensuremath{<}0.001)  & (test=231.11, p\ensuremath{<}0.001) & (test=15.41, p\ensuremath{<}0.001)  & (test=70.85, p\ensuremath{<}0.001) & --                     & --            \\
 UiAutomator       & (test=76.30, p\ensuremath{<}0.001)  & (test=-106.72, p\ensuremath{<}0.001) & (test=71.18, p\ensuremath{<}0.001)  & (test=-81.68, p\ensuremath{<}0.001)  & (test=133.03, p\ensuremath{<}0.001) & (test=-30.14, p\ensuremath{<}0.001) & (test=5.50, p\ensuremath{<}0.001)  & (test=-79.21, p\ensuremath{<}0.001) & --            \\
\hline
\end{tabular}


==> results/table_welchsttest_tap.tex <==
\begin{tabular}{llllllllll}
\hline
                   & Human                  & AndroidViewClient       & Appium                  & Calabash                & Espresso              & Monkeyrunner           & PythonUiAutomator      & Robotium              & UiAutomator   \\
\hline
 Human             & --                     & --                      & --                      & --                      & --                    & --                     & --                     & --                    & --            \\
 AndroidViewClient & (test=45.32, p\ensuremath{<}0.001)  & --                      & --                      & --                      & --                    & --                     & --                     & --                    & --            \\
 Appium            & (test=131.03, p\ensuremath{<}0.001) & (test=162.45, p\ensuremath{<}0.001)  & --                      & --                      & --                    & --                     & --                     & --                    & --            \\
 Calabash          & (test=70.28, p\ensuremath{<}0.001)  & (test=68.78, p\ensuremath{<}0.001)   & (test=-101.84, p\ensuremath{<}0.001) & --                      & --                    & --                     & --                     & --                    & --            \\
 Espresso          & (test=1.63, p=0.114)   & (test=-277.67, p\ensuremath{<}0.001) & (test=-227.34, p\ensuremath{<}0.001) & (test=-170.10, p\ensuremath{<}0.001) & --                    & --                     & --                     & --                    & --            \\
 Monkeyrunner      & (test=32.02, p\ensuremath{<}0.001)  & (test=-6.76, p\ensuremath{<}0.001)   & (test=-114.94, p\ensuremath{<}0.001) & (test=-40.94, p\ensuremath{<}0.001)  & (test=50.00, p\ensuremath{<}0.001) & --                     & --                     & --                    & --            \\
 PythonUiAutomator & (test=11.01, p\ensuremath{<}0.001)  & (test=-97.63, p\ensuremath{<}0.001)  & (test=-194.19, p\ensuremath{<}0.001) & (test=-120.43, p\ensuremath{<}0.001) & (test=29.31, p\ensuremath{<}0.001) & (test=-34.50, p\ensuremath{<}0.001) & --                     & --                    & --            \\
 Robotium          & (test=11.22, p\ensuremath{<}0.001)  & (test=-6.89, p\ensuremath{<}0.001)   & (test=-52.01, p\ensuremath{<}0.001)  & (test=-19.44, p\ensuremath{<}0.001)  & (test=11.46, p\ensuremath{<}0.001) & (test=-4.48, p\ensuremath{<}0.001)  & (test=7.26, p\ensuremath{<}0.001)   & --                    & --            \\
 UiAutomator       & (test=6.36, p\ensuremath{<}0.001)   & (test=-109.51, p\ensuremath{<}0.001) & (test=-199.81, p\ensuremath{<}0.001) & (test=-128.45, p\ensuremath{<}0.001) & (test=14.62, p\ensuremath{<}0.001) & (test=-40.21, p\ensuremath{<}0.001) & (test=-10.49, p\ensuremath{<}0.001) & (test=-9.27, p\ensuremath{<}0.001) & --            \\
\hline
\end{tabular}

